MixFairFace: Towards Ultimate Fairness via MixFair Adapter in Face Recognition

Although significant progress has been made in face recognition, demographic bias still exists in face recognition systems. For instance, it usually happens that the face recognition performance for a certain demographic group is lower than the others. In this paper, we propose MixFairFace framework to improve the fairness in face recognition models. First of all, we argue that the commonly used attribute-based fairness metric is not appropriate for face recognition. A face recognition system can only be considered fair while every person has a close performance. Hence, we propose a new evaluation protocol to fairly evaluate the fairness performance of different approaches. Different from previous approaches that require sensitive attribute labels such as race and gender for reducing the demographic bias, we aim at addressing the identity bias in face representation, i.e., the performance inconsistency between different identities, without the need for sensitive attribute labels. To this end, we propose MixFair Adapter to determine and reduce the identity bias of training samples. Our extensive experiments demonstrate that our MixFairFace approach achieves state-of-the-art fairness performance on all benchmark datasets.

==> Sup/fig/fig_globalface.tex <==
\begin{figure*}[thb]
    \centering
    \includegraphics[width=\textwidth]{Sup/src/globalface.pdf}
    \caption{\textbf{(a)} The identity FPR (iFPR) distributions of different approaches trained on Globalface. The iFPR is sorted from the highest to lowest on RFW identities, and we only show the top 500 identities with the largest FPR. Our framework can significantly reduce the performance variances between the highest and lowest iFPRs, and thus we can achieve the lowest identity bias. \textbf{(b)} The inter-identity similarity distributions of different approaches trained on Globalface. The density of our framework is the largest one, which indicates that the inter-identity similarity variances between identities are the most balanced.}
    \label{fig:sup-globalface}
\end{figure*}

==> Sup/sec/Evaluations.tex <==
\section{Evaluation Protocols}
\input{Sup/tab/tab_balancedface.tex}
\input{Sup/tab/tab_globalface.tex}
\input{Sup/fig/fig_globalface.tex}

As addressed in our main paper, we found that the previous evaluation protocol highly underestimates demographic bias between identities, and the provided verification pairs for testing only cover a small ratio of the entire dataset. In our proposed evaluation protocol, we traverse all pair-wise combinations in the dataset for testing. We first introduce the notations for describing a given dataset, and then we detail the calculation of our proposed metrics.

\paragraph{Notations.}
Given a datasets providing $N$ facial images, $M$ attributes (e.g., $M=4$ for RFW), and $G$ identities (e.g., $G=12,000$ for RFW). We use $\{I_i\}_{i=1}^N$ to denote all images, and the corresponding identity indexes are denoted as $\{y_i\}_{i=1}^N$. The corresponding attribute (e.g., race or skintone) of each image are denoted as $\{a_i\}_{i=1}^N$.

\paragraph{Pair-wise Cosine Similarity.} 
We firstly use our trained networks to extract the feature vector with 512 dimensions $\{f_i\}_{i=1}^N$, $f_i \in \mathbb{R}^{512}$ from all provided facial images. We calculate the cosine similarities of every pair-wise combinations in the dataset, and we denote the cosine similarity of all pairs as $\{S_{i,j} = \cos(f_i, f_j)\}_{i,j=1}^N$. For the pairs in which both images are from the same identity, we define them as positive pairs, while the others are defined as negative ones:
\begin{equation}
    c_{i,j} = \left\{\begin{array}{lr}
            1 & y_i = y_j~,\\
            0 & y_i \neq y_j~.
        \end{array}\right.~,
\end{equation}
where $c_{i,j}$ indicates if a pair is positive or not. 

\paragraph{Overall TPR/FPR.} 
Given a verification threshold $T_u$, the true/false positive and negative cases are defined as:
\begin{equation}
    \begin{aligned}
        \label{eq:tpfptnfn}
        TP_{i,j} &= \delta(S_{i,j}>T_u) \cdot \delta(c_{i,j}=1)~,\\
        FP_{i,j} &= \delta(S_{i,j}>T_u) \cdot \delta(c_{i,j}=0)~,\\
        TN_{i,j} &= \delta(S_{i,j}<T_u) \cdot \delta(c_{i,j}=0)~,\\
        FN_{i,j} &= \delta(S_{i,j}<T_u) \cdot \delta(c_{i,j}=1)~,
    \end{aligned}
\end{equation}
where $\delta$ is a binary function to indicate if a condition is satisfied or not:
\begin{equation}
    \delta(\text{cond}) = \left\{\begin{array}{ll}
        1 & \text{if cond is true}~,\\
        0 & \text{otherwise}~.
    \end{array}\right.~. \\
\end{equation}
With Equation~\eqref{eq:tpfptnfn}, we can calculate the overall average TPR and FPR:
\begin{equation}
    \begin{aligned}
        TPR^* &= \frac{\sum_{i=1}^N \sum_{j=1,j \neq i}^N TP_{i,j}}{\sum_{i=1}^N \sum_{j=1,j \neq i}^N TP_{i,j}+FN_{i,j}}~,\\
        FPR^* &= \frac{\sum_{i=1}^N \sum_{j=1,j \neq i}^N FP_{i,j}}{\sum_{i=1}^N \sum_{j=1,j \neq i}^N FP_{i,j}+TN_{i,j}}~,
    \end{aligned}
\end{equation}
where $TPR^*$ and $FPR^*$ are overall TPR and FPR, respectively.

Considering that a low false positive rate (FPR) is necessary for face recognition systems, we find the verification threshold $T_u$ under a chosen overall FPR. In this paper, we choose 1e-5 as the overall FPR, which is reasonable for face recognition systems.

\paragraph{Attribute-based TPR/FPR.}
The aTPR and aFPR in Table 2 and 3 of our main paper are our proposed attribute-based metrics. Specifically, this metric is calculated for the identities that are in the same attributes, we use this metric to evaluate the performance variances between different races/skinetones. The metric is established as:
\begin{equation}
    \begin{aligned}
        aTPR^t &= \frac{\sum_{i=1}^N \sum_{j=1,j \neq i}^N \delta(a_i = t) \cdot TP_{i,j}}{\sum_{i=1}^N \sum_{j=1,j \neq i}^N \delta(a_i = t) \cdot (TP_{i,j}+FN_{i,j})}~,\\
        aFPR^t &= \frac{\sum_{i=1}^N \sum_{j=1,j \neq i}^N \delta(a_i = t) \cdot FP_{i,j}}{\sum_{i=1}^N \sum_{j=1,j \neq i}^N \delta(a_i = t) \cdot (FP_{i,j}+TN_{i,j})}~,
    \end{aligned}
\end{equation}
where $t$ indicates the attribute index. For RFW dataset, we have four attributes, while there are six attributes for IJB-C~\cite{IJB-C}. We then use the average and standard deviation calculated from $\{aTPR^t\}_{t=1}^M$ and $\{aFPR^t\}_{t=1}^M$ as our attribute-based fairness performance, which are ``Avg'' and ``Std'' in Table 2-4 of our main paper.

\paragraph{Identity-based TPR/FPR.}
We use the proposed identity-based metric to evaluate the performance variances across different identities. We define the identity TPR and FPR as:
\begin{equation}
    \begin{aligned}
        iTPR^k = \frac{\sum_{i=1}^N \sum_{j=1,j \neq i}^N \delta(y_i=k) \cdot TP_{i,j}}{\sum_{i=1}^N \sum_{j=1,j \neq i}^N \delta(y_i=k) \cdot (TP_{i,j}+FN_{i,j})}~,\\
        iFPR^k = \frac{\sum_{i=1}^N \sum_{j=1,j \neq i}^N \delta(y_i=k) \cdot FP_{i,j}}{\sum_{i=1}^N \sum_{j=1,j \neq i}^N \delta(y_i=k) \cdot (FP_{i,j}+TN_{i,j})}~,
    \end{aligned}
\end{equation}
where $k$ indicates the index of identities. ``iFPR-std'' in Table 2-4 of our main paper is the standard deviation calculated from $\{iFPR^k\}_{k=1}^G$. Since the variances of iFPR are much larger than iTPR, we use ``iFPR-std'' to represent the identity bias.

==> Sup/sec/Experiments.tex <==
\section{Experimental Results}

In our supplementary experiments, we provide the results of the 12,000 verification pairs provided by RFW~\cite{RFW}. In addition, we include the figures of identity FPR and inter-identity similarity distributions trained on Globalface~\cite{rl-rbn}.

\subsection{Results of Provided Pairs}
We show experimental results trained on Balancedface and Globalface in Table \ref{tab:sup-balancedface} and \ref{tab:sup-globalface}, respectively. In general, the performance differences between CosFace, CIFP, and our proposed framework are small, but CIFP has the lowest standard deviation. In Table~\ref{tab:sup-balancedface}, we found the accuracy of African from our framework is better than Asian, while the accuracy of African is the worst from the other baselines. However, the provided pairs cannot well represent fairness as addressed in Section 3 of our main paper since the provided pairs are not fairly selected.

\subsection{iFPR Distribution (Globalface)}
We show the iFPR distribution trained on Globalface in Figure~\ref{fig:sup-globalface} (a). Similar to Figure 5 of our main paper, we reduce the difference between the highest and lowest iFPRs, which shows that we reduce the performance inconsistency across identities. 

\subsection{Inter-Identity Similarity (Globalface)}
We show the inter-identity similarity distribution trained on Globalface in Figure~\ref{fig:sup-globalface} (b). Our approach can achieve a more compact distribution, which shows that we can reduce the inter-identity similarity variances between identities and thus achieve the lowest identity bias.

In general, The results trained both Balancedface and Globalface provide a conclusion that our MixFairFace can alleviate the identity bias, i.e., reduce the performance inconsistency between identities, and we can achieve ultimately fair performance while avoiding the fairness skewness issue.

==> Sup/sec/Outline.tex <==
\section{Outline}
In this supplementary materials, we include the following contents:
\begin{enumerate}
    \item Mathematical definitions of attribute-based and identity-based metrics.
    \item Experimental results of the verification pairs provided by RFW.
    \item iFPR and inter-identity similarity distributions trained on Globalface~\cite{rl-rbn}.
\end{enumerate}

\noindent We detail the contents in the following sections.

==> Sup/tab/tab_balancedface.tex <==
% Table generated by Excel2LaTeX from sheet 'previouseval'
\begin{table*}[t]
  \centering
  \caption{The performance of the provided 12,000 verification pairs trained on Balancedface~\cite{rl-rbn}.}
    \begin{tabular}{|r|cccc|cc|}
    \hline
    \textbf{Method} & \textbf{African} & \textbf{Asian} & \textbf{Caucasian} & \textbf{Indian} & \textbf{Avg} & \textbf{Std} \bigstrut\\
    \hline
    \hline
    \textbf{CosFace~\cite{wang2018cosface}} & 94.1  & 94.2  & 96.3  & 94.8  & 94.9  & 1.01 \bigstrut[t]\\
    \textbf{PASS~\cite{pass}} & 87.8  & 89.6  & 92.2  & 90.3  & 90.0  & 1.82 \\
    \textbf{CIFP~\cite{cifp}} & 94.4  & 94.8  & 96.6  & 95.3  & 95.3  & 0.96 \\
    \textbf{Ours} & 94.2  & 93.8  & 96.1  & 95.3  & 94.9  & 1.05 \bigstrut[b]\\
    \hline
    \end{tabular}%
  \label{tab:sup-balancedface}%
\end{table*}%


==> Sup/tab/tab_globalface.tex <==
% Table generated by Excel2LaTeX from sheet 'previouseval'
\begin{table*}[t]
  \centering
  \caption{The performance of the provided 12,000 verification pairs trained on Globalface~\cite{rl-rbn}.}
    \begin{tabular}{|r|cccc|cc|}
    \hline
    \textbf{Method} & \textbf{African} & \textbf{Asian} & \textbf{Caucasian} & \textbf{Indian} & \textbf{Avg} & \textbf{Std} \bigstrut\\
    \hline
    \hline
    \textbf{CosFace~\cite{wang2018cosface}} & 94.4  & 94.8  & 97.5  & 95.8  & 95.6  & 1.38 \bigstrut[t]\\
    \textbf{PASS~\cite{pass}} & 91.2  & 92.5  & 94.9  & 93.1  & 92.9  & 1.54 \\
    \textbf{CIFP~\cite{cifp}} & 94.6  & 95.5  & 97.5  & 95.9  & 95.9  & 1.21 \\
    \textbf{Ours} & 94.5  & 95.0  & 97.3  & 96.1  & 95.7  & 1.24 \bigstrut[b]\\
    \hline
    \end{tabular}%
  \label{tab:sup-globalface}%
\end{table*}%


==> fig/fig_compare1.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{src/compare1.png}
    \caption{The identity FPR (iFPR) distributions of different approaches on Balancedface and Globalface training protocols. The iFPR is sorted from the highest to lowest on RFW identities, and we only show the top 500 identities with the largest FPR. Our MixFairFace significantly reduces the range between the lowest and highest FPR and thus we can achieve the smallest identity bias (iFPR-std).}
    \label{fig:compare1}
\end{figure*}

==> fig/fig_compare2.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{src/compare2.png}
    \caption{The inter-identity similarity distributions of different approaches on Balancedface and Globalface training protocols. Our MixFairFace achieves the largest density, i.e., the similarities of identities are closer than the other baselines. Thus, our approach can largely reduce the identity bias.}
    \label{fig:compare2}
\end{figure*}


==> fig/fig_inter_sim_dist.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\textwidth]{src/distribution.png}
    \caption{(a) The identity FPR (iFPR) distributions of different approaches on Balancedface and Globalface training protocols. The iFPR is sorted from the highest to lowest on RFW identities, and we only show the top 500 identities with the largest FPR. Our MixFairFace significantly reduces the range between the lowest and highest FPR and thus we can achieve the smallest identity bias (iFPR-std). (b) The inter-identity similarity distributions of different approaches on Balancedface and Globalface training protocols. Our MixFairFace achieves the largest density, i.e., the similarities of identities are closer than the other baselines. Thus, our approach can largely reduce the identity bias.}
    \label{fig:inter-sim-dist}
\end{figure}

